CigTime: Corrective Instruction Generation Through Inverse Motion Editing

Recent advancements in models linking natural language with human motions have shown significant promise in motion generation and editing based on instructional text. Motivated by applications in sports coaching and motor skill learning, we investigate the inverse problem: generating corrective instructional text, leveraging motion editing and generation models. We introduce a novel approach that, given a user's current motion (source) and the desired motion (target), generates text instructions to guide the user towards achieving the target motion. We leverage large language models to generate corrective texts and utilize existing motion generation and editing frameworks to compile datasets of triplets (source motion, target motion, and corrective text). Using this data, we propose a new motion-language model for generating corrective instructions. We present both qualitative and quantitative results across a diverse range of applications that largely improve upon baselines. Our approach demonstrates its effectiveness in instructional scenarios, offering text-based guidance to correct and enhance user performance.

==> sections/temp.tex <==
\section{Goal}


\subsection{Task}



In this work, we tackle the problem of motion correction tasks. Intuitively, motion correction can be understood as such a task. We assume a trainer and a trainee, with the trainee attempting to perform a certain type of action. The trainer knows the ideal state of that action, observes the trainee's action, and provides feedback for modifications. The trainee then adjusts their action based on the feedback to meet the trainer's requirements for that type of action. From the perspectives of the trainee and the trainer, we need to accomplish two distinct subtasks: 

\paragraph{Motion correctional instruction generation. \yyc{make sure this term is aligned with the literature, e.g., why not correctional motion instruction generation?} \fqh{It is aligned with PoseFix where use pose correctional rather than correctional pose.}}
For the trainer, they need to compare the trainee's motion with the ideal motion to provide feedback for improvement.
Formally, this task takes a source motion sequence $m^{s} \in \mathbb{R}^{T \times J}$, where $T$ is the number of frames and $J$ is the dimensionality of the motion representation,  and a target motion sequence $m^t$ as input and aims  to learn a function $\mathcal{T}$ which can map $m^s$ and $m ^ t$ to the correction text instruction $l$, $\mathcal{T}(m^s, m^t) = l$
\yyc{define ``edit $m^s$ to $m^t$,'' suggestion, you can define the above tasks more clearly by instantiating mappings, i.e., $\phi$ or $\psi$}



\paragraph{Text-based motion editing.} 
For the trainee, they need to be able to adjust their motion based on correctional instructions.
Formally, Given a source motion sequence 
$m^{s} $,  and a correctional text instruction $l$, 
the goal of the text-based motion editing task is to learn another function $\mathcal{S}$ which can map $m^s$ and $l$ to target motion sequence $m^t$, $\mathcal{S}(m^s, l) = m^t$.
\yyc{explicitly state the output of text-based motion editing, i.e., define the task by a clear definition of the output.}



\yyc{after reading your task definitions, if these are the tasks you are aiming for, you have to come up with a unified task name and definition, e.g., task A, and to accomplish task A, a pipeline should be able to do ``text-based motion editing'' and ''correctional instruction generation.'' Otherwise, readers will be unsure of what you are trying to do}



\subsection{Data Collection}

Most of the existing related datasets \cite{guo2022generating,lin2024motion} concentrate on the annotation for a single motion sequence. These datasets ignore the correlations between different motion sequencces and may assign similar or even sane annotation to multiple different motion sequences. This makes them unsuitable for application in motion correction tasks.
\yyc{this sentence does not convey why since you are also focusing on text-to-motion or motion annotation, first say out the difference between the tasks that existing focus on and your task} 

Some works build correctional instruction datasets by rule-based methods. 
However, they are designed for specific actions and always require expert experience and careful tuning to design the rules. 

Recently, PoseFix proposed to utilize pre-defined codes to represent the difference between two poses. Since motion data introduces changes over time, this makes the variations between two different motion sequences more difficult to characterize and express compared to the variations between poses. 

However, compared with static pose, motion sequence involves temporal variations. Comparing two motion sequences requires us to extract the temporal features of both sequences and align the two sequences. This exceeds the problem scope that PoseFix is capable of solving.
%Simply applying PoseFix to motion data would result in redundant and inefficient information, as shown in Fig \ref{}. 
\yyc{what do you mean by redundant and inefficient information, this is not defined so far}. 

Thus, to tackle the problem of motion correction, we need to construct a dataset that includes source-target motion pairs and corresponding instructions.
%it is important to create a correctional instruction dataset for general actions to  
\yyc{do not use we think, use objective facts that make the creation of a new dataset obvious, also you have to define the so called dataset before you state you are going to create one.}
%We assume that the source motion sequence $m^s$ and target motion sequence $m^t$ have similar appearance and perform similar tasks \yyc{similar semantic meaning is a very vague word, change it, e.g., sequences performing similar tasks?}, otherwise describing the difference between $m^s$ and $m^t$ is almost equivalent to describing $m^t$ itself \yyc{what do you mean by this sentence, not even sure what equivalent means in this way}.
To acquire the triplet data combined by $m^s$, $m^t$, and $l$, we collect the motion sequences from different sources and design two methods to annotate the correctional instructions.

\paragraph{Motion data collection.}

Our goal is to obtain motion sequence pairs that have similar appearances or perform similar actions and correctional instruction annotations that describe the differences between them. Thus, we collect motion pairs with similar appearance or semantic meanings from three sources. These three sources collect data from existing datasets, generated data, and internet videos, increasing the size and diversity of the dataset.
\yyc{after reading the following, i got a more clear idea of how you are going to collect the data, but you have to state at the beginning why you resort to the following options, what are the reasonings? convince the reviewer that besides the following options, we do not have a better option.  }:
\begin{itemize}
    \item \textbf{From existing dataset.} Some existing datasets, such as Fit3d, 3DYoga90, and Flag3D are created with 3D motion sequence and action category annotation while each category has more than one motion sequence. From these datasets, we can easily collect motion pairs with similar appearances and semantic meanings and split them into source motions and target motions.

    \item \textbf{Generated by pre-trained model.} Most of the existing motion generation models are stochastic, which means we can generate different motion sequences corresponding to the same instruction. Thus, it is also possible to utilize pretraining generation models to generate motion pairs. However, these methods can not guarantee that they can generate correct motions corresponding to the input instruction. Thus, we need to manually check the generated motions and filter out the pairs without similar appearances.

    \item \textbf{Collect data from Internet}.  We are also interested in collecting data from internet videos. In some sports videos, certain actions are often repetitively performed by multiple times. For example, in tennis videos, we may see multiple serve or forehand hits. These repetitive actions always have similar appearances. To extract the repetitive motions, we run the motion capture method first and then utilize BID to recognize and segment each action clip. Similar to generated data, the quality of estimated motion is always poor. Thus, we still need to manually check these motions and filter out the low-quality pairs.
\end{itemize}


\paragraph{Correctional instruction data collection.}

We still hope to manually annotate some data that better reflects human language habits. However, when we attempted to give the collected motion pairs to humans for labeling, we found that their annotations often lacked some important factors, resulting in poor data quality, as shown in Fig.
\yyc{this reason is too vague, which makes it not a convincing reason}. Addressing this issue, we design a novel pattern for correctional instruction collection. 
To be specific, in this data collection process, we need a trainer and a trainee to help us complete data collection. The trainee \yyc{weird name, use a more professional one, e.g., coach and trainee} is assigned source motion sequences to imitate, while another tester the trainee is given target motion sequences. 
\yyc{use the professional names to rewrite the following. can get some inspiration from the game ``Hole in the Wall''}
The trainee imitates the actions from the source motion sequences, and the trainer, who has access to the target motion sequences, observes the trainee's actions and provides correctional instructions to help align the actions closer to those of the target motion sequences.
\yyc{why you want A to imitate the source action first? are there any other options? e.g., B tell A to do a motion, and then corrects?} \fqh{"B tell A to do a motion" does not align with our definition of the task formulation.}
This may involve adjustments in speed, amplitude, direction, or other aspects. The trainee and trainer alternate between performing action corrections based on the provided correctional instructions and giving new correctional instructions as needed \yyc{need to explicitly state what information A receives and what information B receives, this is very important, and also state why!}. 
The process continues until the trainer, who has access to the target motion sequences, believes that the trainee's actions are consistent with the target motion sequences. We integrate multiple rounds of instructions to obtain the final correctional instruction.

The above process can provide correctional instructions that are in line with human language habits and fully express the differences between two motion sequences. However, this process is time-consuming and unscalable. Therefore, we only perform the above process on a small portion of motion pairs. For other motion pairs, we design a new annotation method that prompts LLMs to generate correctional instructions based on given source and target motion sequences. Through this method, we can generate a large amount of data that meets our requirements in zero-shot \yyc{how this is achieved?}. 

To be specific, we first convert each motion sequence $m \in \mathbb{R}^{T \times J}$ to $p \in \mathbb{R}^{T \times K \times 3}$ which represents the 3D positions of the joints, where $K$ is the number of joints.
We first randomly select a frame $p_i \in \mathbb{R}^{K \times 3}$ from the dataset and input it into ChatGPT-4 according to a pre-designed template, enabling it to understand 3D joint positions.
Afterward, we randomly select another frame $p_j \in \mathbb{R}^{K \times 3}$ to input into ChatGPT-4, allowing ChatGPT-4 to attempt to compare the differences in pose between the two frames. During this process, we manually check the outputs of LLMs and provide appropriate reminders when errors occur, until the LLMs can accurately describe the pose of a single frame or the differences between the poses of two frames.

After ChatGPT-4 successfully understands the pose of a single frame or the differences between two frames' poses, we randomly select a motion sequence $m$ and convert it into 3D joint position sequence $p$, sample it at a lower FPS, and input the sampled sequence $p$ into ChatGPT-4 through a template, allowing ChatGPT-4 to attempt to describe this motion sequence. Subsequently, we gradually increase the sampling rate and input it to ChatGPT-4 until it reaches the original FPS of $m$. During this process, we do not correct the output of ChatGPT-4. When the entire process is completed, we input the source motion $m^s$ and target motion $m^t$ to ChatGPT-4 through a pre-designed template, and command it to provide a corrective instruction. Although we do not provide any sequence-level annotations, ChatGPT-4 can still output instructions that match the motion sequences we input.




































\subsection{Model training.}

Although in the above data collection process, we can already output correctional instructions through LLMs. But that requires us to make extensive corrections to the output of LLMs and not fully utilize the data we collect through human interaction. Meanwhile, we found that prompt ChatGPT-4 can only be used to output corrective instructions and cannot be used for text-based motion editing, as ChatGPT-4 always tends to output 3D joint positions with simple patterns and loses a lot of details. Thus, We hope to train a model that can handle both text-based motion editing and motion correctional instruction generation simultaneously.

Fine-tuning pre-trained LLMs has been proven to be an effective solution for multimodal problems. 
Inspired by past work, we design a fine-tuning method for LLMs, enabling them to perform both text-based motion editing and motion correctional instruction generation tasks simultaneously. We divided the entire fine-tuning process into three steps: tokenizing the motion, learning how to complete motion correction tasks, and further optimizing the results using high-quality data.
\yyc{why do you call it fine-tuning?}. \fqh{Because LLMs are pre-trained.}

\yyc{without stating what you are trying to achieve, I have difficulties in understanding the following.}
\paragraph{Step 1.} We apply a VQ-VAE-like structure to convert the input motion sequences into discrete tokens. To be specific, we utilize an encoder $\mathcal{E}$ to map the input motion sequence $m$ into a continuous feature $f \in \mathbb{R}^{T \times D}$, where $D$ is the dimensionality of the continuous feature. 
\begin{equation}
\label{eq:encoding}
f = \mathcal{E}(m), \text { where } f \in \mathbb{R}^{T \times D}.
\end{equation}

The codebook $c \in \mathbb{R}^{K \times D}$ represents different action flow fields, where $K$ is a predefined number of different discrete codes or motion modes and $c_k \in \mathbb{R}^D$ is the k-th action representation. 
The VQ layer encodes the sequence feature $f$ to a discrete latent code(s) $z  \in  \mathbb{R}^{T \times D}$ through codebook $c$ by projecting each per-frame feature $f_i$ to its nearest code:
\begin{equation}
VQ\left(f_i\right)=c_k, \text { where } k=\operatorname{argmin}_j\left\|f_i-c_j\right\|_2^2,
\end{equation}
where $VQ$ represents the VQ layer, $Z$ is the ensemble $\{VQ(f_i)\}_{i=1}^{T}$, and $k$ is the code index.

Before we get the discrete codes $z$, we
utilize a decoder to decode $z$ into $m'$. We exploit reconstruction loss between $m$ and $m'$ and commit loss for supervision.

\yyc{fully lost.}


\paragraph{Step 2.} In this step, we aim to fine-tune the pre-trained LLM model Vicuna-16B for our tasks. \yyc{what is a vicuna-16B, what does it do, input output and why you want to fine tune it? for what?}. \fqh{Vicuna-16B is a pre-trained LLM model, we explain why we need to fine-tune a pre-trained LLM model above.}

For the text-based motion edition task, we feed $m^s$ and $m^t$ into our pre-training encoder $\mathcal{E}$ and utilize codebook $c$ to get the discrete feature $z^s$ and $z^t$ \yyc{this is different from what you told me? i remember you have no trained encoder at all, just predefined rules?}. \fqh{I guess you mean the data collection pipeline which has been discussed above by "what I told you".} We use the pre-defined input template to combine the $z^s$ with the correctional instruction $l$ \yyc{what does this instruction mean?} \fqh{Correctional instruction. I use the same nouns to express the same concepts.} as the input of a LLM $\mathcal{L}$ and use the output template to convert $z^t$ as the ground truth of the output of $\mathcal{L}$  \yyc{what is this LLM? what is its input and what is its output? DEFINITION! Also, you are using a template, can be treated as rule based, but you mention that previous rule based is not good, but you did not state why yours is better.} \fqh{Firstly, this LLM refers to pre-trained Vicuna-16B. Secondly, defining the input and output is exactly what this paragraph is doing. Or should I write it like $\mathcal{L}(z^s, l)=z^t$? Finally, I cannot understand why a template can be treated as rule-based. I think there is a significant misalignment between us.}


For the correctional instruction generation task, we utilize a template to convert $z^s$ and $z^t$ as the input and utilize the instruction $l$ as the ground truth of the output of $\mathcal{L}$.\yyc{totally lost, do not know what you are trying to do there} \fqh{Definite the input and output for correction instruction generation task. }

\paragraph{Step 3.} 
Considering that the amount of data we annotate through humans is small but of high quality, we will perform an additional fine-tuning process for this data. This process is consistent with the description in Step 2, but we only use human-annotated data for fine-tuning.
\yyc{how? what is the connection with the previous one} 
\fqh{Same process, but only use human-annotated data}

\fqh{Again, I think there is a significant misalignment between us. Perhaps it's because my previous version didn't clearly state what to do at the beginning of this section, or maybe it's because of my poor writing skills. But in these two paragraphs, almost all of your questions were raised just after the answers, which is a bit strange.}





\subsection{Evaluation metrics}
Existing NLP evaluation metrics are not adequate for semantic assessment and may not ensure that the correctional instruction output by a model can drive a trainee from $m^s$ to $m^e$. 
To validate the instruction output from the model at the semantic level for motion correctional instruction generation task, we design one novel user-study method. 
Similar to data collection, we provide source motion sequences and target motion sequences to a trainer and a trainee. In addition, we provide instructions to the trainee who has previously received source motion sequences and ask them to correct their motion based on the instructions \yyc{very vague so far, e.g., what do you mean by correct their motion on their own? why this is meaning? to make the evaluation make sense, you have to first tell us what metrics you want to check and why they are important to check}. The trainer who receives target motion sequences needs to determine whether the trainee's motion is the same as the motion they receive. 
We use the probability of the trainee successfully performing the target motion sequences as an evaluation metric.

\yyc{lost without understanding anything here. rewrite!}

\subsection{Contribution}
1. Dataset
2. Utilize LLMs for zero-shot correctional instruction generation.
3. Novel data collet and evaluation metric.


{\color{red} PUT your math symbol definitions in the preamble. Start working on it now.}

The method section of a research paper also referred to as the methodology or materials and methods section, should include the following elements:

1. Research design: Begin by describing the overall research design or approach you used to address your research question or problem. This could include experimental, quasi-experimental, correlational, descriptive, qualitative, quantitative, or mixed-methods designs.

2. Participants or subjects: Provide details about the population or sample you studied, including the number of participants, demographics, and any relevant selection or recruitment criteria. Explain how the participants were chosen, addressing issues such as random sampling or convenience sampling.

3. Materials or instruments: Describe any materials, instruments, or tools used in your study, such as questionnaires, surveys, interview protocols, or apparatus for conducting experiments. Provide details on the reliability and validity of these instruments, if applicable.

4. Procedures: Outline the step-by-step procedures followed in your research, including data collection and data analysis methods. Be clear and detailed so that other researchers can replicate your study if needed. If your study involved multiple phases or components, describe each part separately.

5. Data analysis: Explain the statistical or qualitative data analysis techniques used to analyze your data. This could include descriptive statistics, inferential statistics, content analysis, or thematic analysis, among others. Mention any software programs used in the analysis process, if applicable.

6. Ethical considerations: Describe the ethical considerations and procedures followed in your study, such as obtaining informed consent, ensuring confidentiality and anonymity, or addressing potential risks to participants. If your study required approval from an Institutional Review Board (IRB) or ethics committee, mention this as well.

7. Limitations: Acknowledge any limitations of your methods, such as potential biases, sampling issues, or constraints that may affect the generalizability or validity of your findings. Discuss how you addressed or mitigated these limitations where possible.

The method section should be clear, concise, and detailed enough to allow other researchers to understand and potentially replicate your study. It demonstrates the rigor and validity of your research by providing a transparent account of how you conducted your investigation.
